Cloth-Splatting: 3D Cloth State Estimation from RGB Supervision

We introduce Cloth-Splatting, a method for estimating 3D states of cloth from RGB images through a prediction-update framework. Cloth-Splatting leverages an action-conditioned dynamics model for predicting future states and uses 3D Gaussian Splatting to update the predicted states. Our key insight is that coupling a 3D mesh-based representation with Gaussian Splatting allows us to define a differentiable map between the cloth state space and the image space. This enables the use of gradient-based optimization techniques to refine inaccurate state estimates using only RGB supervision. Our experiments demonstrate that Cloth-Splatting not only improves state estimation accuracy over current baselines but also reduces convergence time.

==> sections/old/01_Introduction.tex <==
\section{Introduction}
\todoinr{Formulate contributions}

% Motivation: estimating the state of cloths is hard. Object-level representations are not enough, but imposing a deformation-aware representation faces perceptual challenges. Robot often perceives these objects thorugh vision, and extractin the 3D state of the cloth is limited by the high dimensional state space and self-occlusion.

Object-centric 3D representations have recently shown impressive results in achieving few-shot learning for manipulation, due to their potential to improve generalization and sim-to-real transfer over traditional image representations \cite{huang2022mesh, wang2023one}. The spatial awareness of these representations, often augmented with semantic descriptors, offers strong transfer capabilities to diverse variations of object properties and environment settings. However, when it comes to deformable such as clothes, object-centric representations do not necessarily contain enough information about the state of the cloth due to the infinite degrees of freedom these objects have. Ideally, 3D state representations of cloth should be deformation aware, where this awareness comes from spatial or semantic structural priors. However, due to the complex dynamics, infinite dimensional state-space, and self-occlusion, estimating such representation is still an open problem. 

% What other people propose - 3D representation
A common way to describe cloth states using 3D representations is either through graphs or point clouds. However, the unordered nature of point clouds hinders geometry awareness due to self-occlusions, making it difficult to distinguish between different layers of the cloth when being folded~\cite{longhini2024adafold}. Graph-based representations, while theoretically capable of capturing the underlying structure of the cloth under occlusions, prove difficult to be effectively used in real-world scenarios due to the challenges of tracking the deformation~\cite{longhini2022edo,huang2023self}. The tracking problem leads to poor 3D state estimation.
% Semantics not really explored


% What we propose

In this work we propose \modelname. a vision-supervised 3D state estimation of cloths. Our method combines \ac{gs} and action-conditioned dynamics priors to estimate the cloth deformations and update the state estimate from RGB observations. The key insight is that \ac{gs} serves as a differentiable map from the state space of the cloth to the observation space, which is then leveraged to update the state estimate analogously to a filtering approach. To further enable few-shot learning from demonstration, we augment the 3D representation to achieve deformation awareness with two inductive biases: mesh structure and semantic descriptors.

% What we show
We showcase how our state estimation approach leads to more accurate 3D state estimation of cloth. Its filtering nature allows for the refinement of inaccurate estimations of novel-real world cloth for which the action-conditioned model falls short. We further show that our state estimation enables learning manipulation policies from one demonstration that transfer to different objects of the same category and different object poses. 

% contributions

In summary, our contributions are:
\begin{itemize}
    \item A mesh-constrained object-centring extension of \ac{gs}.
    \item A vision-supervised 3D state estimation for cloth with action-conditioned dynamics priors.
\end{itemize}




==> sections/old/02_RW.tex <==
\section{Related Work}

\begin{itemize}
    \item Cloth state estimation and modeling
    \item Cloth tracking in the real world
    \item Cloth manipulation from demonstration
\end{itemize}

\subsection{Cloth Representation}
\todoing{Fuse cloth representation and modelling}

A common way to describe cloth states is using 3D representations such as graphs or point clouds due to their potential to improve generalization and sim-to-real transfer over traditional image representations \cite{huang2022mesh, wang2023one}. However, point clouds are often ambiguous due to self-occlusions, making it difficult to distinguish between different layers of the cloth when being folded~\cite{longhini2024adafold}. Graph-based representations, while theoretically capable of capturing the underlying structure of the cloth under occlusions, prove difficult to be effectively used in real-world scenarios due to the challenges of tracking the deformation~\cite{longhini2022edo,huang2023self}.
\al{Discuss more in detail the challenges of state estimation in real-world settings based on different representations. }

\al{If more general in the representation, we could include DINOBot}


\subsection{Cloth Modeling}
Approaches to model clothes can be divided into two categories: physics-based and data-driven methods.

Physics-based approaches utilize classical mechanics to model cloth deformations, involving steps like internal forces computation, collision detection, and response. While delivering realistic simulations suitable for various garments, they often fall short in real-time applications like virtual try-ons due to high computational demands. Innovations aim to enhance speed and efficiency using techniques like GPU acceleration and parameter estimation from video data, yet challenges in setup speed and computational efficiency persist.

Data-driven models harness data to learn how garments deform under external forces, e.g., human body or manipulation actions. Techniques involve training with 3D meshes derived from various sources and using neural networks to accelerate deformation computations. While promising, these methods struggle with garment topology changes and require substantial data, limiting their adaptability to new garment types without retraining. Graph-based methods such as GNN emerge as a promising approach to model dynamic clothing motions through advanced techniques like multi-level message passing. These methods provide enhanced generalization across different simulations and address the propagation challenges inherent in graph-based systems, setting a new standard for modeling dynamic garment motions.

\al{Add a discussion about using simulation to model the dynamics like other gaussian splatting papers.}


\subsection{Cloth Tracking}
\al{This could be more general in terms of tracking objects, with one paragraph describing the compiter vision community and then one smaller paragraph describing what has been done in robotics}


\subsection{Few-shot Learning from Demonstrations}

Few-shot learning from demonstration can be divided into two fundamental approaches: behavioral cloning and feature correspondences. Behaviour Cloning relies on a neural network trained over a dataset of observation-action pairs coming from an expert demonstrator. This method often requires hundreds of laborious demonstrations to learn tasks. Feature correspondences 


One-shot imitation learning (Abbeel)

Task-embedded control networks for few-shot imitation
learning. 


 Transporter networks: Rearranging the visual world for
robotic manipulation. 

Learning to rearrange deformable cables, fabrics, and bags with goal-conditioned transporter
networks.

SPARSEDFF: SPARSE-VIEW FEATURE DISTILLATION FOR ONE-SHOT DEXTEROUS MANIPULATION (DINOv2. Policy learne as keypoint matching

Learning Generalizable Manipulation Policies with Object-Centric 3D Representations (DINOv2r) but it is just for object segmentation. The policy is learned as BC and on an action trajectory. We focus instead on a pick and place, and what we have to learn is an heat-map for the pick and one for the place.

Dense object nets: Learning dense visual object descriptors by and for robotic manipulation.

Self-supervised correspondence in visuomotor policy learning.

kpam: Keypoint affordances for categorylevel robotic manipulation

Unsupervised learning of object keypoints for perception and control.

The surprising effectiveness of representation learning for visual imitation,

\subsection{Vision-based dynamics estimation}
\todoing{Include dynamic NerF}
\todoing{Include dynamic Gaussians}
\todoing{Include few physics inspired things}
\todoing{Include keypoint trackers}


\todoino{Optional: Maybe include table which aggregates information from the different domains (graphics, robotics, vision)}

==> sections/old/03_P_Formulation.tex <==
\section{Problem Formulation}

\todoing{Use mesh instead of graph and update the document}
\todoing{Remove Kalman Filter-or find better analogy}
\todoing{Replace focus on tracking with focus on state estimation}
\todoing{Improve notation of images and camera matrices}

The problem is estimating the 3D state of a cloth when undergoing deformation due to an external force, given a set of multi-view RGB(-D) images $I^P_{t}$ at timestep $t \in [0,\ldots,H]$ with corresponding camera matrices $P$. 

We describe the state of the cloth at time $t$ using a simulation mesh $M_t = (V, E)$ with nodes $V$ connected by edges $E$. The nodes $V = {v_i}_{i=1...N}$ represent the particles that compose the cloth, where $v_i = (x_i, \dot{x}_i)$ denotes the particle’s current position and velocity, respectively.
We consider two types of edges $E$ in the graph, representing two types of interactions: mesh edges and action edges. The mesh edges $E^M$ characterize interactions between particles, where we consider a triangular mesh to define the connectivity structure. Each edge $e_{ij} = (v_i , v_j ) \in E_M$ connects nodes $v_i$ to $v_j$ and models the mesh connection between them. The action edges $E^A$ instead specify interactions between the cloth particles and external forces, such as a robot or a human picking a corner of the cloth and applying a force to lift it. This external force is defined as an acceleration applied to all the grasped particles of the cloth. 

We cast the problem of tracking as an optimization problem ... 
We formulate the problem of state estimation for cloth manipulation in a manner analogous to a Kalman filter. Our goal is to estimate the state of a cloth, represented as a 3D mesh, over time. The state of the cloth at time $t+1$ is predicted through a transition function $f$, conditioned on robot actions. Mathematically, the state transition can be expressed as:
\[
\hat{M}_{t+1} = f(\hat{M}_t, a_t)
\]
where $\hat{M}_t$ denotes the estimated state of the cloth at time $t$, and $a_t$ represents the robot actions affecting the cloth between times $t$ and $t+1$.

The only available observation at each time step is the RGB image of the cloth, derived from an emission map $w$. This map transforms the state of the cloth, represented in the graph domain, into the RGB domain:
\todoing{Improve formulation to iterate over all the observed images}
\[
I^P_t = w(\hat{M}_t, P) 
\]
where $z_t$ is the observed RGB image at time $t$.


% \todoing{Understand what to do with this part - Method or not?}

% To enhance generalizability across different cloth sizes, poses, and object categories, we introduce a feature map $s$ that elevates the 3D vertices of the cloth mesh to a higher-dimensional space of semantic features. These features are designed to be equivariant to transformations such as translations and rotations, and adaptable across different objects:
% \[
% \phi(x_t) = s(\hat{x}_t)
% \]
% where $\phi(x_t)$ represents the semantically enriched feature representation of the cloth state.





==> sections/old/04_Method.tex <==
\section{Method}


\todoing{Add figure of our method. Any idea how to visualize it?}

In a standard Bayesian filtering approach, the update step incorporates the new observation to refine the state estimate. Analogously, we aim to update our 3D state estimation using the observed RGB data. However, in real-world applications, we often lack an accurate, action-conditioned transition function and a well-defined emission map. Therefore, we utilize a data-driven model to approximate the transition function $f$, and employ Gaussian Splatting for the emission function $w$, which allows for differentiable rendering of the 3D state.
\begin{itemize}
    \item 1) Learn a dynamics model as state estimation
    \item 2) Mesh-constrained Gaussian Splatting as emission map
    \item 3) Photometric loss with residual learning as update.
\end{itemize}

\subsection{Action-conditioned Cloth Dynamics}

\todoing{Coordinate the mesh terminology}
\todoing{describe the methodology fully}
\todoing{Shrink and move to the appendix the full}

For simulating the cloth, we use a \ac{gnn} $f_\theta$ defined by the parameters $\theta$:
\begin{equation}
  \hat{G}^{t+1} = f_\theta(G^t, G^{t-1},\ldots, G^{t-k}, a^t)\text{.}
\end{equation}
The GNN receives a sequence of the last $k$ states of the mesh and the external forces $a^t$ affecting the system.
These forces can be passive such as gravity or active such as a robotic action manipulating the cloth.
The goal is then to simulate the cloth to find a prediction for the next cloth state $\hat{G}^{t+1}$, which in practice means predicting the next positions $\hat{x}^{t+1}_p$.


\subsection{Gaussian Splatting (estimation)}
\label{subsec:estimation}
\todoing{Split in emission function desctiption and fine-tuning description}
In the estimation step, the predicted state of the mesh $\hat{G}^{t}$ is used to render an image via Gaussian Splatting.
This is done by projecting the Gaussians' positions $x^t_p$ and covariances $\Sigma^t_p$ to the image plane and then using $\alpha$-blending to aggregate their colors $c_p$ to pixel colors.
This allows for supervising the position of the Gaussians, i.e.~the positions of the vertices in the mesh, via an image reconstruction loss:

\begin{equation}
w(\tilde{M}^{t} = \hat{M}^{t} + \Delta M(t), P)
\end{equation}


\begin{equation}
    \mathcal{L}_{rgb} = || I^t_{P} - w(\tilde{M}^{t} ||^2_2 \text{.}
\end{equation}
In addition to the image reconstruction, we intend to use additional regularisation terms $\mathcal{L}_{reg}$ based on expected physical properties of cloth \cite{grigorev2023hood}.
The loss is then used to iteratively find an improved estimate for the mesh state $\tilde{G}^{t}$ i.e. the positions $\hat{x}^t_p$, therefore solving the tracking problem.
\al{This needs to be extended especially in the case where we learn the delta dynamics}
\mb{Add barycentric representation}
\mb{Add projective function for GS}

\subsection{Cloth Manipulation via Feature Matching}
\al{Missing the description of the "bag" of demonstrations.}

Actions $\{ a_j\}_{j=1}^n$ are pick and place coordinates such that $a_j = (x_{\text{pick}},x_{\text{place}} )$, pixels if in the image space, or 3D positions in the task space.  The robot grasps the world coordinates associated
with the grasp point and then moves to the world coordinates
associated with the place point without changing the end
effector orientation. The robot is provided with one demonstrations of pick and places that might require $n$ steps. $\{ a_j\}_{j=1}^n$, and  $\{ O_j\}_{j=1}^n$, where $O$ is the observation which can be again either images or different 3D cloth representations.   At test-time, a similar (flattened) object is dropped onto the surface, and the goal is to generate a corresponding sequence of actions for this object that imitate the given demonstration. Specifically, 


\[
\{a^*_j\}^n_{j=1} = \{\argmin (d_{O_j,O'_j}(x_{\text{pick}})), \argmin (d_{O_j,O'_j}(x_{\text{place}}))\}^n_{j=1}
\]
for $j \in \{1,\ldots,n\}$ where $d_{O_j,O'_j} \colon \mathbb{R}^2 \to \mathbb{R}^2$ is a function which estimates the corresponding point $x'_{\text{pick}}$ in $O'$ given a point $x_{\text{pick}}$ in $O$. This function is difficult to compute in the image space where the texture changes, which is why we seek different features describing the state of the cloth. In practice, assume that you have a better way of extracting descriptors from the observations by defining a map $f_0: O \rightarrow F$ from observation space to feature space. Then, the distance can be computed in the feature space. Then, the best action can be found by minimizing the correspondence function:
\[
(x'_{\text{pick}},x'_{\text{place}} ) = \arg \min_{(x_{\text{pick}},x_{\text{place}} )} \| f_0(O_j, (x_{\text{pick}},x_{\text{place}} )) - f_0(O', (x'_{\text{pick}},x'_{\text{place}} )) \|^2 
\]


The first equation computes the top matching keypoint based on their distance in descriptor space.


\subsection{Color/feature Diffusion Algorithm}

Required definitions:
\begin{itemize}
  \item Let $ G = (V, E) $ be a graph where $ V $ is the set of vertices and $ E $ is the set of edges.
  \item The adjacency matrix $ A $of $ G $is defined such that $ A_{ij} = 1 $ if there is an edge between nodes $ i $and $ j $, and $ A_{ij} = 0 $ otherwise.
  \item The degree matrix $ D $i s a diagonal matrix where each diagonal element $ D_{ii} $ is the degree of node $ i $, i.e., the number of edges connected to node $ i $.
  \item The graph Laplacian $ L $ is defined as $ L = D - A $.
\end{itemize}


Let $ \mathbf{u}(t) \in \mathbb{R}^{n \times 3} $ represent the colors of the $ n $ nodes at time $ t $, where each row corresponds to the RGB color values of a node. The diffusion of colors across the graph can be modeled using the Laplacian matrix to update the colors over time. The update rule in discrete time can be written as:
\[
\mathbf{u}(t+1) = \mathbf{u}(t) - \epsilon L \mathbf{u}(t)
\]
Where  $ \epsilon $is a small scalar representing the step size of the diffusion process, and $ t $indexes the time step.
We would like some keypoint nodes \al{define} to have fixed colors that do not change over time, representing boundary conditions in the diffusion process. If $ \mathcal{C} $is the set of nodes with fixed colors, then for all $ i \in \mathcal{C} $and for all $ t $:
\[
\mathbf{u}_i(t+1) = \mathbf{u}_i(0)
\]
Where $ \mathbf{u}_i(0) $are the initial color values of the nodes in $ \mathcal{C} $. The diffusion steps updated the color values according to the diffusion equation until convergence or for a fixed number of iterations \al{define better the convergence criteria based on the cloth dimension. Probably, we want to use as a parameter the diameter of the graph}




==> tables/tracking.tex <==
% \begin{tabular}{lcccccc}
% \toprule
%  \textbf{Method}    &    \texttt{SHORTS-1} &   \texttt{SHORTS-2} &   \texttt{TOWEL} &  \texttt{TSHIRT-1} &   \texttt{TSHIRT-2} & Mean\\ \midrule
% \rowcolor{lavender}
% \multicolumn{7}{c}{3D MTE [mm] $\downarrow$} \\ 
% \midrule
% RAFT Oracle \cite{teed2020raft} & 5.34 & 33.304 & 29.07 & 3.128 & 3.92 & 14.952   \\
% DynaGS \cite{dyna3dgs} & 5.081 &         10.624 &         6.627 &          6.409 &          8.678  & 7.483 \\
% MD-Splatting \cite{duisterhof2023mdsplatting}&  5.815 &         10.970 &        10.457 &          4.387 &          5.77  & 7.479 \\
% GNN & 4.006 &         21.552 &         5.755 &          4.061 &          6.458 & 8.366 \\
% \modelname{} (Ours)  &          \textbf{1.882} &          \textbf{8.923} &         \textbf{2.110}  &          \textbf{0.940}  &          \textbf{2.058}  & \textbf{3.182} \\
% \midrule
% \rowcolor{lavender}
% \multicolumn{7}{c}{3D $\delta_{avg}$ $\uparrow$} \\
% \midrule
% RAFT Oracle \cite{teed2020raft} & 0.72 & 0.56 & 0.507 & 0.82 & 0.658 & 0.652  \\
% DynaGS \cite{dyna3dgs} &  0.858 &          0.744 &         0.786 &          0.88  &          0.807 & 0.815 \\
% MD-Splatting \cite{duisterhof2023mdsplatting}&  0.871 &          0.761 &         0.750  &          0.891 &          0.847 & 0.824 \\
% GNN &  0.840  &          0.663 &         0.843 &          \textbf{0.925} &          0.848 & 0.823 \\
% \modelname{} (Ours)  & \textbf{0.874} &          \textbf{0.786} &         \textbf{0.852} &          0.906 &          \textbf{0.871} & \textbf{0.857} \\
% \midrule
% \rowcolor{lavender}
% \multicolumn{7}{c}{3D Survival Rate $\uparrow$} \\
% \midrule
% RAFT Oracle \cite{teed2020raft} & 0.672 & 0.512 & 0.516 & 0.803 & 0.647 & 0.630 \\
% DynaGS \cite{dyna3dgs}& 0.838 &          0.704 &         0.736 &          0.885 &          0.775 & 0.787 \\
% MD-Splatting \cite{duisterhof2023mdsplatting}& 0.868 &          0.708 &         0.694 &          0.879 &          0.805 & 0.790  \\
% GNN & 0.813 &          0.622 &         0.801 &          \textbf{0.906} &          0.821 & 0.792 \\
% \modelname{} (Ours)   & \textbf{0.871} &          \textbf{0.749} &         \textbf{0.819} &          0.867 &          \textbf{0.830} & \textbf{0.827} \\
% \bottomrule
% \label{tab:main_results}
% \end{tabular}

\begin{tabular}{llcccccc}
\toprule
 \textbf{Metric}    &  \textbf{Method}    &    \footnotesize{\texttt{SHORTS-1}} &   \footnotesize{\texttt{SHORTS-2}} &   \footnotesize{\texttt{TOWEL}} &  \footnotesize{\texttt{TSHIRT-1}} &   \footnotesize{\texttt{TSHIRT-2}} & Mean\\ \midrule
% \midrule
\multirow{5}{*}{\shortstack[l]{3D MTE \\  ~~$\downarrow$ $[\text{mm}]$ }}                          &RAFT-Oracle \cite{teed2020raft} & 5.340 & 33.304 & 29.07 & 3.128 & 3.920 & 14.952   \\
 ~                          &DynaGS \cite{dyna3dgs} & 5.081 &         10.624 &         6.627 &          6.409 &          8.678  & 7.483 \\
 & MD-Splatting \cite{duisterhof2023mdsplatting}&  5.815 &         10.970 &        10.457 &          4.387 &          5.770  & 7.479 \\
 ~                          &GNN & 4.006 &         21.552 &         5.755 &          4.061 &          6.458 & 8.366 \\
 ~                          &\modelname{}  &          \textbf{1.882} &          \textbf{8.923} &         \textbf{2.110}  &          \textbf{0.940}  &          \textbf{2.058}  & \textbf{3.182} \\
% \midrule
% \rowcolor{lavender}
% \multicolumn{7}{c}{3D $\delta_{avg}$ $\uparrow$} \\
\midrule
 \multirow{5}{*}{\shortstack[l]{3D $\delta_{avg}$ \\  $~~~~\uparrow$ }}                           & RAFT-Oracle \cite{teed2020raft} & 0.720 & 0.560 & 0.507 & 0.82 & 0.658 & 0.652  \\
 ~                          & DynaGS \cite{dyna3dgs} &  0.858 &          0.744 &         0.786 &          0.880  &          0.807 & 0.815 \\
        &MD-Splatting \cite{duisterhof2023mdsplatting}&  0.871 &          0.761 &         0.750  &          0.891 &          0.847 & 0.824 \\
 ~                          & GNN &  0.840  &          0.663 &         0.843 &          \textbf{0.925} &          0.848 & 0.823 \\
 ~                          & \modelname{}  & \textbf{0.874} &          \textbf{0.786} &         \textbf{0.852} &          0.906 &          \textbf{0.871} & \textbf{0.857} \\
% \midrule
% \rowcolor{lavender}
% \multicolumn{7}{c}{3D Survival Rate $\uparrow$} \\
\midrule
 \multirow{5}{*}{\shortstack[l]{Survial \\ ~~~rate \\  $~~~~\uparrow$ }}                             &RAFT Oracle \cite{teed2020raft} & 0.672 & 0.512 & 0.516 & 0.803 & 0.647 & 0.630 \\
~                          &DynaGS \cite{dyna3dgs}& 0.838 &          0.704 &         0.736 &          0.885 &          0.775 & 0.787 \\
  & MD-Splatting \cite{duisterhof2023mdsplatting}& 0.868 &          0.708 &         0.694 &          0.879 &          0.805 & 0.790  \\
~                          &GNN & 0.813 &          0.622 &         0.801 &          \textbf{0.906} &          0.821 & 0.792 \\
~                          &\modelname{}   & \textbf{0.871} &          \textbf{0.749} &         \textbf{0.819} &          0.867 &          \textbf{0.830} & \textbf{0.827} \\
\bottomrule
\label{tab:main_results}
 \vspace{-25pt}
\end{tabular}
